Dynamic Regret Minimization for Control of Non-stationary Linear Dynamical Systems

We consider the problem of controlling a Linear Quadratic Regulator (LQR) system over a finite horizon $T$ with fixed and known cost matrices $Q,R$, but unknown and non-stationary dynamics $\{A_t, B_t\}$. The sequence of dynamics matrices can be arbitrary, but with a total variation, $V_T$, assumed to be $o(T)$ and unknown to the controller. Under the assumption that a sequence of stabilizing, but potentially sub-optimal controllers is available for all $t$, we present an algorithm that achieves the optimal dynamic regret of $\tilde{\mathcal{O}}\left(V_T^{2/5}T^{3/5}\right)$. With piece-wise constant dynamics, our algorithm achieves the optimal regret of $\tilde{\mathcal{O}}(\sqrt{ST})$ where $S$ is the number of switches. The crux of our algorithm is an adaptive non-stationarity detection strategy, which builds on an approach recently developed for contextual Multi-armed Bandit problems. We also argue that non-adaptive forgetting (e.g., restarting or using sliding window learning with a static window size) may not be regret optimal for the LQR problem, even when the window size is optimally tuned with the knowledge of $V_T$. The main technical challenge in the analysis of our algorithm is to prove that the ordinary least squares (OLS) estimator has a small bias when the parameter to be estimated is non-stationary. Our analysis also highlights that the key motif driving the regret is that the LQR problem is in spirit a bandit problem with linear feedback and locally quadratic cost. This motif is more universal than the LQR problem itself, and therefore we believe our results should find wider application.

==> buffer.tex <==
\textbf{Bounding the total length of bad intervals:} By definition of bad intervals, we can bound $\size{\cI^\bad \cap \cI}$, the total number of time periods within bad intervals within an arbitrary interval $\cI$ by:
\begin{align}
\label{eqn:size_bad_int}
    \size{\cI^\bad \cap \cI } & = \sum_{t \in \cI^\bad \cap \cI} 1 \leq \sum_{t \in \cI^\bad \cap \cI} \frac{2}{C_3} \min\left\{ \norm{ \hat{\Theta}_t - {\Theta}_t}_F^2  , C_3\right\} \leq \frac{2}{C_3} \sum_{t \in \cI} \min\left\{ \norm{ \hat{\Theta}_t - {\Theta}_t}_F^2 , C_3 \right\}.
    \end{align} 


The bulk of the work will be in bounding $T_4$ through the the following regret decomposition for good intervals.
